Data Augmentation Alone Can Improve Adversarial Training

Adversarial training suffers from the issue of robust overfitting, which seriously impairs its generalization performance. Data augmentation, which is effective at preventing overfitting in standard training, has been observed by many previous works to be ineffective in mitigating overfitting in adversarial training. This work proves that, contrary to previous findings, data augmentation alone can significantly boost accuracy and robustness in adversarial training. We find that the hardness and the diversity of data augmentation are important factors in combating robust overfitting. In general, diversity can improve both accuracy and robustness, while hardness can boost robustness at the cost of accuracy within a certain limit and degrade them both over that limit. To mitigate robust overfitting, we first propose a new crop transformation, Cropshift, which has improved diversity compared to the conventional one (Padcrop). We then propose a new data augmentation scheme, based on Cropshift, with much improved diversity and well-balanced hardness. Empirically, our augmentation method achieves the state-of-the-art accuracy and robustness for data augmentations in adversarial training. Furthermore, when combined with weight averaging it matches, or even exceeds, the performance of the best contemporary regularization methods for alleviating robust overfitting. Code is available at: https://github.com/TreeLLi/DA-Alone-Improves-AT.

==> tables/padcrop-cropshift.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[]
\centering
\caption{Performance of variants of our augmentation}
\label{tab: padcrop cropshift}
\begin{tabular}{@{}llllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{SWA}} &
  \multicolumn{1}{c}{\multirow{2}{*}{Augmentation}} &
  \multicolumn{3}{c}{Accuracy (\%)} &
  \multicolumn{3}{c}{Robustness (\%)} \\ \cmidrule(l){3-8} 
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{} &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} \\ \midrule
\multirow{2}{*}{w.o.} &
  ours-padcrop &
  83.74 &
  84.82 &
  -1.09 &
  50.15 &
  49.25 &
  0.90 \\
 &
  ours-cropshift &
  {\ul \textbf{83.96}} &
  {\ul \textbf{84.92}} &
  {\ul \textbf{-0.97}} &
  {\ul \textbf{50.74}} &
  {\ul \textbf{49.99}} &
  {\ul \textbf{0.75}} \\ \midrule
\multirow{2}{*}{w.} &
  ours-padcrop &
  83.11 &
  85.21 &
  {\ul \textbf{-2.10}} &
  51.14 &
  49.40 &
  {\ul \textbf{1.74}} \\
 &
  ours-cropshift &
  {\ul \textbf{84.18}} &
  {\ul \textbf{86.45}} &
  -2.27 &
  {\ul \textbf{51.73}} &
  {\ul \textbf{49.88}} &
  1.85 \\ \bottomrule
\end{tabular}
\end{table}

==> tables/reg-robustness_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[tbp]
\centering
\caption{Performance of methods for alleviating robust overfitting for PreAct ResNet18 on CIFAR10 (assessed using PGD10 and AA). 
The source of the result is noted if copied from another work, otherwise, it is determined by us. 
All methods use the same training setting, except RST due to the use of unlabeled data, is trained for the equivalent of 400 epochs, twice many as used for others.}
\label{tab: regularization methods robustness}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}llllllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Method}} &
  \multicolumn{3}{c}{Accuracy} &
  \multicolumn{3}{c}{PGD10} &
  \multicolumn{3}{c}{AA} \\ \cmidrule(l){2-10} 
\multicolumn{1}{c}{} &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} \\ \midrule
baseline &
  82.50 &
  83.99 &
  -1.49 &
  53.35 &
  46.01 &
  7.34 &
  48.21 &
  42.46 &
  5.75 \\
RST \citep{rice_overfitting_2020} &
  82.80 &
  77.00 &
  {\ul \textbf{5.80}} &
  {\ul \textbf{59.80}} &
  52.90 &
  6.90 &
  - &
  - &
  - \\
AWP \citep{yu_understanding_2022}$^1$ &
  82.00 &
  81.11 &
  0.89 &
  - &
  - &
  - &
  49.94 &
  49.69 &
  {\ul \textbf{0.25}} \\
MLCAT \citep{yu_understanding_2022}&
  84.10 &
  84.77 &
  -0.67 &
  - &
  - &
  - &
  50.70 &
  50.32 &
  0.38 \\
CONS \citep{tack_consistency_2022} &
  {\ul \textbf{85.25}} &
  {\ul \textbf{86.45}} &
  -1.20 &
  - &
  - &
  - &
  49.05 &
  48.57 &
  0.48 \\
KD &
  84.51 &
  85.40 &
  -0.89 &
  - &
  - &
  - &
  49.87 &
  49.72 &
  0.15 \\
TE \citep{dong_exploring_2022}&
  82.35 &
  82.79 &
  -0.44 &
  55.79 &
  54.83 &
  {\ul \textbf{0.96}} &
  50.59 &
  49.62 &
  0.97 \\
% ours-weak &
%   84.98 &
%   85.82 &
%   -0.84 &
%   55.28 &
%   53.54 &
%   1.74 &
%   50.34 &
%   48.94 &
%   1.40 \\
IDBH[strong] (ours) &
  83.96 &
  84.92 &
  -0.97 &
  55.65 &
  54.67 &
  0.98 &
  50.74 &
  49.99 &
  0.75 \\
IDBH[weak]+SWA (ours)&
  84.18 &
  {\ul \textbf{86.45}} &
  -2.27 &
  57.10 &
  54.32 &
  2.79 &
  {\ul \textbf{51.73}} &
  49.88 &
  1.85 \\
IDBH[strong]+SWA (ours) &
  82.98 &
  85.49 &
  -2.51 &
  56.84 &
  {\ul \textbf{55.60}} &
  1.24 &
  51.49 &
  {\ul \textbf{50.77}} &
  0.72 \\ \bottomrule

\end{tabular}%
}
{\footnotesize$^1$\citet{yu_understanding_2022} reported the robustness without accuracy, so the accuracy is copied from \citet{wu_adversarial_2020}}
\end{table}


==> tables/svhn-tin.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[tbp]
\centering
\caption{Accuracy and robustness of the baseline and our augmentations on SVHN and TIN.}
\label{tab: svhn tin}
\begin{tabular}{@{}llllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Dataset}} &
  \multirow{2}{*}{Augmentation} &
  \multicolumn{3}{c}{Accuracy (\%)} &
  \multicolumn{3}{c}{Robustness (\%)} \\ \cmidrule(l){3-8} 
\multicolumn{1}{c}{} &
   &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} \\ \midrule
\multirow{2}{*}{SVHN} & baseline & 90.55 & 90.18 & 0.37  & 47.48 & 40.86 & 6.62 \\
                      & ours     & 93.70 & 93.92 & -0.21 & 54.56 & 54.09 & 0.46 \\ \midrule
\multirow{2}{*}{TIN}  & baseline & 46.94 & 46.60 & 0.34  & 20.19 & 13.82 & 6.37 \\
                      & ours     & 50.88 & 50.76 & 0.12  & 21.36 & 19.04 & 2.32 \\ \bottomrule
\end{tabular}%
\end{table}

\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llllllll@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Dataset}} &
  \multirow{2}{*}{Augmentation} &
  \multicolumn{3}{c}{Accuracy (\%)} &
  \multicolumn{3}{c}{Robustness (\%)} \\ \cmidrule(l){3-8} 
\multicolumn{1}{c}{} &
   &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} &
  \multicolumn{1}{c}{best} &
  \multicolumn{1}{c}{end} &
  \multicolumn{1}{c}{diff.} \\ \midrule
\multirow{2}{*}{SVHN} & baseline & 90.55 & 90.18 & 0.37  & 47.48 & 40.86 & 6.62 \\
                      & ours     & 93.70 & 93.92 & -0.21 & 54.56 & 54.09 & 0.46 \\ \midrule
\multirow{2}{*}{TIN}  & baseline & 46.94 & 46.60 & 0.34  & 20.19 & 13.82 & 6.37 \\
                      & ours     & 50.88 & 50.76 & 0.12  & 21.36 & 19.04 & 2.32 \\ \bottomrule
\end{tabular}%
}
